MD-split+: Practical Local Conformal Inference in High Dimensions

Quantifying uncertainty in model predictions is a common goal for practitioners seeking more than just point predictions. One tool for uncertainty quantification that requires minimal assumptions is conformal inference, which can help create probabilistically valid prediction regions for black box models. Classical conformal prediction only provides marginal validity, whereas in many situations locally valid prediction regions are desirable. Deciding how best to partition the feature space X when applying localized conformal prediction is still an open question. We present MD-split+, a practical local conformal approach that creates X partitions based on localized model performance of conditional density estimation models. Our method handles complex real-world data settings where such models may be misspecified, and scales to high-dimensional inputs. We discuss how our local partitions philosophically align with expected behavior from an unattainable conditional conformal inference approach. We also empirically compare our method against other local conformal approaches.

==> sections/background.tex <==


\david{6/22 first draft done, feel free to edit and add}

A fundamental goal in predictive inference is to build a prediction region for a test point $(\X_{n+1},Y_{n+1})$ given training data $(\X_1,Y_1),\ldots,(\X_n,Y_n)$, with all data drawn i.i.d. from the same distribution. Here, $\X \in \mathbb{R}^d$ denotes covariates or features, $Y \in \mathbb{R}$ denotes a response variable, and we will use $\widehat C_n(\X_{n+1}) \subseteq \mathbb{R}$ to denote the prediction region for $Y_{n+1}$ given $\X_{n+1}$. Without assumptions on the data-generating distribution, it is challenging to obtain valid uncertainty quantification$-$that is, to ensure that $Y_{n+1} \in \widehat C_n(\X_{n+1})$ with probability at least $1 - \alpha$ for some nominal $\alpha \in [0,1]$.

There are multiple notions of what the above statement means. For example, one may wish $Y_{n+1} \in \widehat C_n(\X_{n+1})$ to hold with probability $1-\alpha$ at every point $\X_{n+1}=\x$, or only on average over the distribution of $\X_{n+1}$. More formally, we define these notions as \textit{conditional coverage} and \textit{marginal coverage}, respectively. Let $P$ denote a joint probability distribution on $(\X,Y) \in \mathbb{R}^d \times \mathbb{R}$.

\begin{Definition}[\textbf{Conditional Coverage}]
\label{def:cond_cov}
    A method for generating prediction regions $\widehat C_n$ achieves distribution-free conditional coverage at level $1-\alpha$ if
    \begin{align}
    \label{eq:cond_cov}
        \pr \left( \left\{ Y_{n+1} \in \widehat C_n(\X_{n+1}) \Big| \X_{n+1} = \x \right\} \right) \geq 1-\alpha
    \end{align}
    for all distributions $P$ and almost all $\x$.
\end{Definition}

\begin{Definition}[\textbf{Marginal Coverage}]
\label{def:cond_cov}
    A method for generating prediction regions $\widehat C_n$ achieves distribution-free marginal coverage at level $1-\alpha$ if
    \begin{align}
    \label{eq:cond_cov}
        \pr \left( \left\{ Y_{n+1} \in \widehat C_n(\X_{n+1}) \right\} \right) \geq 1-\alpha
    \end{align}
    for all distributions $P$.
\end{Definition}

\david{6/25 We need to describe split conformal - structurally we rely on this. Maybe there's a better way to present this?}
One well known strategy for distribution-free predictive inference is the split conformal method \citep{Papadopoulos2002, Vovk2013, Lei2018}, which splits the training data into two subsets, $\mathcal{D}_1 = \{(\X_1,Y_1),\ldots,(\X_l,Y_l)\}$ and $\mathcal{D}_2 = \{(\X_m,Y_m),\ldots,(\X_m,Y_m)\}$, where $l+m=n$. $\mathcal{D}_1$ is used to train a method for generating a \textit{conformal score}, $g: \mathcal{X} \times \mathcal{Y} \to \mathbb{R}$, which is then computed over $\mathcal{D}_2$ to obtain what are called split residuals, $\{U_i = g(\X_i,Y_i)\}_{i=1}^m$. Because $g$ is constructed in such a way that the split residuals are i.i.d. given $g$, the rank of $U_{n+1}$ is uniform among $\{1,\ldots,m+1\}$. It follows that $\widehat C_n(X_{n+1}) = \left\{y: g(\X_{n+1},y) \geq U_{\lfloor \alpha \rfloor} \right\}$ is a prediction region that achieves level $(1-\alpha)$ marginal coverage:
\begin{align*}
    \pr(U_{n+1} \geq U_{\lfloor \alpha \rfloor}) \geq 1-\alpha \\
    \pr(g(\X_{n+1},Y_{n+1}) \geq U_{\lfloor \alpha \rfloor}) \geq 1-\alpha \\
    \pr\left(Y_{n+1} \in \left\{y: g(\X_{n+1},y) \geq U_{\lfloor \alpha \rfloor} \right\} \right) \geq 1-\alpha 
\end{align*}
where $U_{\lfloor \alpha \rfloor}$ denotes the $\alpha$-quantile (or the $\lfloor m\alpha \rfloor$-th order statistic) among $U_1,\ldots,U_{m+1}$. 

In practice, stronger guarantees than marginal coverage may be desirable, as it is possible for coverage to be high on average across a population while being inadequate for entire subgroups. It is known that distribution-free methods cannot achieve conditional coverage, unless one imposes strong assumptions on the distribution $P$ \citep{Vovk2013, Lei2014, Barber2019a}. Fortunately, it is possible to obtain coverage guarantees intermediate between marginal and conditional coverage, that offer ``approximately'' conditional coverage. For instance, we can define the notion of local coverage.

\begin{Definition}[\textbf{Local Coverage}]
\label{def:cond_cov}
    A method for generating prediction regions $\widehat C_n$ achieves distribution-free local coverage at level $1-\alpha$ if
    \begin{align}
    \label{eq:cond_cov}
        \pr \left( \left\{ Y_{n+1} \in \widehat C_n(\X_{n+1}) \Big| \X_{n+1} \in A \right\} \right) \geq 1-\alpha
    \end{align}
    for all distributions $P$ and all $A \in \A$, where $\A$ is a partition of $\mathcal{X}$.
\end{Definition}

With an appropriate partition $\A$, a method that satisfies local coverage can guarantee that coverage is high across all subgroups of interest. One can adapt the split conformal idea to achieve local coverage by adaptively changing the cutoff, $U_{\lfloor m\alpha \rfloor}$, depending on the value of $X_{n+1}$. In particular, one could compute $U_{\lfloor m\alpha \rfloor}$ using only the points $\X_i$ in $\mathcal{D}_2$ that belong to the same partition element of $\A$ as the observed $X_{n+1}$. A key question, then, is how to select $\A$. One method is to simply partition $\mathcal{X}$ based on Euclidean distance \citep{Lei2014, guan2019localconf}. But this does not scale well to high-dimensional settings, because it is difficult to create partition elements that are large enough to contain sufficiently many observations $\X_i$, while remaining small enough to still offer ``local'' or ``approximately'' conditional coverage.

Another approach is to train a conditional density estimator (CDE), denoted $\widehat f(y|\x)$, on the data, and to take $\widehat f$ as the conformal score function $g$ \citep{Izbicki2020,Izbicki2021}. One then places observations $X_i$ and $X_j$ in the same partition based on how similar their estimated densities are, which may be a more natural grouping than Euclidean distance. This approach has the advantage of scaling to high dimensions, as well as allowing for non-contiguous prediction regions. However, to be successful, this method crucially relies on the assumption that $\widehat f$ is consistent. That is, there must exist $\eta_n = o(1)$ and $\rho_n = o(1)$ such that
\begin{align}
    \label{assump:f_consistent}
    \pr \left( \E \left[ \sup_{y\in\mathcal{Y}} \left( \widehat f(y|\x) - f(y|\x) \right)^2 \Big| \widehat f \right] \geq \eta_n \right) \leq \rho_n
\end{align}

\add{TODO: add CD-split+ description (and other relevant Izbicki stuff; not sure if HPD stuff is relevant)}

In practice, however, CDEs $\widehat f(y|\x)$ may be misspecified and inconsistent, especially in situations that call for larger, more complex models. Moreover, in finite sample settings, there is no guarantee that $\widehat f$ is a good approximation for $f$.

Recently, there have been diagnostics developed for validating the quality of fit of CDEs locally in the feature space $\mathcal{X}$ \citep{zhao2021diagnostics}. Given a CDE model $\widehat f$ and an observed point $(\x,y)$, we define highest predictive density (HPD) values \citep{diana2015hpd} as follows:
\begin{align}
    \label{eq:HPD}
    \HPD(\y; \x) = \int_{{\y'}:\widehat{f}({\y'} | \x) \geq \widehat{f}(\y | \x)} \widehat{f}({\y'} | \x) d{\y'}
\end{align}
$\HPD(\y; \x)$ is a measure of how plausible $\y$ is according to $\widehat f(\y|\x)$, with small values indicating high plausibility. We then define
\begin{align}
    r_{\alpha}(\x) = \pr(\HPD(Y;\x) < \alpha | \x)
\end{align}
as the level $\alpha$ coverage function of the HPD sets, for some $\alpha \in [0,1]$. Note that if $\widehat f = f$, then the HPD values are uniform, which means that $r_{\alpha}(\x) = \alpha$ for any $\alpha \in [0,1]$.

% diagnostic tool, focuses on localized CDE model performance
% though can be used to e.g. test diagnostics to see whether it fits, it provides us with P-P plots that we can use (HPD has beautiful probabilistic interpretations)
% intrinsically philoosphically aligned with confomral inference. if we do HPD with my method, our method is suggesting we have a model, but actually the amount of mass in that HPD level set was not 0.5 but it was 0.6. Conformal inference doe sthe exact same thing. You gave e a sequence of nested sets, and I picked this one to get 1-alpha coverage, but it wasn't necessarily the one you said. If you provide conformal inference with a model that has HPD splits, looking just at a single x and doing a local approach, the model will provide us a seq of nested sets related to conformal score (e.g. HPD values). But conformal inference will say hey, the level set that has the right amount of mass is this one, regarldess of what your HPD values said. Mirroring this, my diagnostic method says hey this is what the actual HPD coverage is.
% tradeoff: need data to fit second rhat models
Given a fixed $\alpha$ and training data $(\X_1,Y_1),\ldots,(\X_n,Y_n)$, we can define $W^{\alpha}_i = \I(\HPD(Y_i;\X_i) < \alpha )$ for $i=1,\ldots,n$. We can then obtain an estimate for $r_{\alpha}$, which we denote $\widehat r_{\alpha}$, by regressing $W_1,\ldots,W_n$ on $\X_1,\ldots,\X_n$. By repeating this process over a grid of values for $\alpha \in [0,1]$, we obtain a ``profile'' of $\{\widehat r_{\alpha}\}$ estimates. Now, at any given location $\x \in \mathcal{X}$ in the feature space, deviations of $\widehat r_{\alpha}(\x)$ from $\alpha$ for various values of $\alpha$ indicate that the CDE model $\widehat f$ does not fit the true conditional density $f$ well. Furthermore, the specific pattern of which values of $\alpha$ are in disagreement, and by how much, form a rough ``signature'' of the specific nature of the distributional deviation of $\widehat f$ from $f$, which we can compute at any location $\x \in \mathcal{X}$.

%\david{6/22 For now, I'm not mentioning asymptotic conditional coverage, because we don't do any theory. Can think about what we want to try to show. For example, \cite{Izbicki2020} showed that empirically, CD-split converges to HPD sets, and he then proved in \cite{Izbicki2021} that converging to HPD sets means achieving asymptotic conditional coverage. Idk if we can do something simple and analogous to this?}



